SuperGaussian: Repurposing Video Models for 3D Super Resolution

We present a simple, modular, and generic method that upsamples coarse 3D models by adding geometric and appearance details. While generative 3D models now exist, they do not yet match the quality of their counterparts in image and video domains. We demonstrate that it is possible to directly repurpose existing (pretrained) video models for 3D super-resolution and thus sidestep the problem of the shortage of large repositories of high-quality 3D training models. We describe how to repurpose video upsampling models, which are not 3D consistent, and combine them with 3D consolidation to produce 3D-consistent results. As output, we produce high quality Gaussian Splat models, which are object centric and effective. Our method is category agnostic and can be easily incorporated into existing 3D workflows. We evaluate our proposed SuperGaussian on a variety of 3D inputs, which are diverse both in terms of complexity and representation (e.g., Gaussian Splats or NeRFs), and demonstrate that our simple method significantly improves the fidelity of the final 3D models. Check our project website for details: supergaussian.github.io

==> 05-discussion.tex <==
\section{Discussion}

==> figures/application.tex <==


\begin{figure}[t]
  \centering
  \footnotesize
  \includegraphics[width=\linewidth]{figures/instant_3D_examples_3}
  % \setlength\tabcolsep{0.1em}
  % % \resizebox{\linewidth}{!}
  % {
  %   \begin{tabular}{ccccc}
  %      \rotatebox{90}{\phantom{spacin}Instant3D} & \includegraphics[width=.24\linewidth]{figures/instant3d/blue_frog_before_crop} 
  %       & \includegraphics[width=.24\linewidth]{figures/instant3d/frog_before_crop} 
  %       & \includegraphics[width=.24\linewidth]{figures/instant3d/mushroom_before_crop} 
  %       & \includegraphics[width=.24\linewidth]{figures/instant3d/fish_before_crop}   \\
  %      \rotatebox{90}{\phantom{spacin}Upsampled} & 
  %      \includegraphics[width=.24\linewidth]{figures/instant3d/blue_frog_after_crop} 
  %       & \includegraphics[width=.24\linewidth]{figures/instant3d/frog_after_crop} 
  %       & \includegraphics[width=.24\linewidth]{figures/instant3d/mushroom_after_crop} 
  %       & \includegraphics[width=.24\linewidth]{figures/instant3d/fish_after_crop} \\ 
  %   \end{tabular}
  % }
  \vspace{-1em}
   \caption{\textbf{Upsampling text-to-3D generation results.} We apply \methodname to outputs generated by Instant3D~\cite{Li2023Instant3D}, a recent state-of-the-art text-to-3D method. Our method upsamples the input triplane-based representations into high-quality Gaussian splats.} 
   \vspace{-1em}
   \label{fig:application_on_aigc}
\end{figure}

==> figures/qual_on_LLFF.tex <==
\begin{table}[t]
  \centering
  \footnotesize
  \includegraphics[width=\linewidth]{figures/LLFF_results.pdf}
  % \vspace{-2em}
  % \setlength\tabcolsep{0.1em}
  % % \resizebox{\linewidth}{!}
  % {
  %   \begin{tabular}{ccccc}
  %      \rotatebox{90}{\phantom{spacin}Instant3D} & \includegraphics[width=.24\linewidth]{figures/instant3d/blue_frog_before_crop} 
  %       & \includegraphics[width=.24\linewidth]{figures/instant3d/frog_before_crop} 
  %       & \includegraphics[width=.24\linewidth]{figures/instant3d/mushroom_before_crop} 
  %       & \includegraphics[width=.24\linewidth]{figures/instant3d/fish_before_crop}   \\
  %      \rotatebox{90}{\phantom{spacin}Upsampled} & 
  %      \includegraphics[width=.24\linewidth]{figures/instant3d/blue_frog_after_crop} 
  %       & \includegraphics[width=.24\linewidth]{figures/instant3d/frog_after_crop} 
  %       & \includegraphics[width=.24\linewidth]{figures/instant3d/mushroom_after_crop} 
  %       & \includegraphics[width=.24\linewidth]{figures/instant3d/fish_after_crop} \\ 
  %   \end{tabular}
  % }
   \captionof{figure}{\textbf{Qualitative comparison on $2\times$ upsampling between ours and baselines. } We compare our method to qualitative results in their Fig. 3 obtained from FastSR-NeRF for direct comparison. For fair comparison, we use TensoRF in the 3D reconstruction step. With off-the-shelf video prior plugged into \methodname, ours produce upsampled results on par with state-of-the-art quality with delicate detail preserved.
   }
   \vspace{-1em}
   \label{fig:qual_comparison_on_llff}
\end{table}

==> figures/qual_over_multi_level_upsampling.tex <==


\begin{table}[t]
  \centering
  \footnotesize
  \setlength\tabcolsep{0.1em}
  % \resizebox{\linewidth}{!}
  {
    \begin{tabular}{ccc}\sffamily
         low-res input &\sffamily $\times 4$ upsampling &\sffamily $\times 16$ upsampling\\
         \includegraphics[width=.24\linewidth]{figures/multi_level_upsampling/dino_25_64x64} 
         & \includegraphics[width=.24\linewidth]{figures/multi_level_upsampling/dino_25_256x256.png}  
        & \includegraphics[width=.24\linewidth]{figures/multi_level_upsampling/dino_25_1024x1024.png}   \\
        \includegraphics[width=.24\linewidth]{figures/multi_level_upsampling/dino_15_64x64.png} 
        & \includegraphics[width=.24\linewidth]{figures/multi_level_upsampling/dino_15_256x256.png} 
        & \includegraphics[width=.24\linewidth]{figures/multi_level_upsampling/dino_15_1024x1024.png} \\ 
        \includegraphics[width=.24\linewidth]{figures/multi_level_upsampling/dino_10_64x64.png} 
        & \includegraphics[width=.24\linewidth]{figures/multi_level_upsampling/dino_10_256x256.png} 
        & \includegraphics[width=.24\linewidth]{figures/multi_level_upsampling/dino_10_1024x1024.png} \\ 
    \end{tabular}
  }
    % \vspace{-1.5em}
   \captionof{figure}{\textbf{Multi-level up-sampling.} While \methodname is designed to perform $\times$4 upsampling, in practice we can achieve high upsampling factors by running our video upsampler iteratively. Rows are results from different poses of the upsampled 3D scene.}
   \label{fig:multi_level_upsampling}
\end{table}

==> figures/qual_over_need_for_fitting_after_restoration.tex <==


\begin{table}[t]
  \centering
  \footnotesize
  \setlength\tabcolsep{0.1em}
  % \resizebox{\linewidth}{!}
  {
    \begin{tabular}{ccccc}
       \rotatebox{90}{\phantom{spacin}w/o recon} & \includegraphics[width=.24\linewidth]{figures/video_fitting_need/type_1_basket.png} 
        & \includegraphics[width=.24\linewidth]{figures/video_fitting_need/type1_broccoli.png} 
        & \includegraphics[width=.24\linewidth]{figures/video_fitting_need/type_1_crab.png} 
        & \includegraphics[width=.24\linewidth]{figures/video_fitting_need/type_1_pineapple.png}   \\
       \rotatebox{90}{\phantom{spacin}w/  recon} & 
       \includegraphics[width=.24\linewidth]{figures/video_fitting_need/type_2_basket.png} 
        & \includegraphics[width=.24\linewidth]{figures/video_fitting_need/type2_broccoli.png} 
        & \includegraphics[width=.24\linewidth]{figures/video_fitting_need/type_2_crab.png} 
        & \includegraphics[width=.24\linewidth]{figures/video_fitting_need/type_2_pineapple.png} \\ 
    \end{tabular}
  }
   \captionof{figure}{\textbf{Ablation on whether to perform 3D reconstruction after each restoration iteration}. 
   }
   \label{fig:need_for_fitting}
\end{table}

==> figures/qual_over_realworld_gaussian.tex <==


\begin{table}[t]
  \centering
  \footnotesize
  \setlength\tabcolsep{0.1em}
  \includegraphics[width=0.8\linewidth]{figures/realworld_gaussian_demo.pdf}
   \captionof{figure}{\textbf{\methodname over real-world captured 3D gaussian splats.} 
   }
   \label{fig:restoration_iteration}
\end{table}

==> figures/qual_over_restoration_iteration.tex <==


\begin{table}[t]
  \centering
  \footnotesize
  \setlength\tabcolsep{0.1em}
  \includegraphics[width=0.6\linewidth]{figures/iterations_ablation}
  % \resizebox{\linewidth}{!}
  % {
  %   \begin{tabular}{cccccc}
  %       iter 0 & iter 1 & iter 2 & iter 3 & iter 4 & iter 5 \\
  %      \includegraphics[width=.16\linewidth]{figures/video_restoration_iterations/basket_iter_0.png} 
  %       & \includegraphics[width=.16\linewidth]{figures/video_restoration_iterations/basket_iter_1.png} 
  %       & \includegraphics[width=.16\linewidth]{figures/video_restoration_iterations/basket_iter_2.png} 
  %       & \includegraphics[width=.16\linewidth]{figures/video_restoration_iterations/basket_iter_3.png}   
  %       & \includegraphics[width=.16\linewidth]{figures/video_restoration_iterations/basket_iter_4.png} 
  %       & \includegraphics[width=.16\linewidth]{figures/video_restoration_iterations/basket_iter_5.png}   \\
  %      \includegraphics[width=.16\linewidth]{figures/video_restoration_iterations/broccoli_iter_0.png} 
  %       & \includegraphics[width=.16\linewidth]{figures/video_restoration_iterations/broccoli_iter_1.png} 
  %       & \includegraphics[width=.16\linewidth]{figures/video_restoration_iterations/broccoli_iter_2.png} 
  %       & \includegraphics[width=.16\linewidth]{figures/video_restoration_iterations/broccoli_iter_3.png} 
  %       & \includegraphics[width=.16\linewidth]{figures/video_restoration_iterations/broccoli_iter_4.png} 
  %       & \includegraphics[width=.16\linewidth]{figures/video_restoration_iterations/broccoli_iter_5.png}   \\
  %       \includegraphics[width=.16\linewidth]{figures/video_restoration_iterations/crab_iter_0.png} 
  %       & \includegraphics[width=.16\linewidth]{figures/video_restoration_iterations/crab_iter_1.png} 
  %       & \includegraphics[width=.16\linewidth]{figures/video_restoration_iterations/crab_iter_2.png} 
  %       & \includegraphics[width=.16\linewidth]{figures/video_restoration_iterations/crab_iter_3.png} 
  %       & \includegraphics[width=.16\linewidth]{figures/video_restoration_iterations/crab_iter_4.png} 
  %       & \includegraphics[width=.16\linewidth]{figures/video_restoration_iterations/crab_iter_5.png}   \\
  %       \includegraphics[width=.16\linewidth]{figures/video_restoration_iterations/pineapple_iter_0.png} 
  %       & \includegraphics[width=.16\linewidth]{figures/video_restoration_iterations/pineapple_iter_1.png} 
  %       & \includegraphics[width=.16\linewidth]{figures/video_restoration_iterations/pineapple_iter_2.png} 
  %       & \includegraphics[width=.16\linewidth]{figures/video_restoration_iterations/pineapple_iter_3.png} 
  %       & \includegraphics[width=.16\linewidth]{figures/video_restoration_iterations/pineapple_iter_4.png} 
  %       & \includegraphics[width=.16\linewidth]{figures/video_restoration_iterations/pineapple_iter_5.png}   \\
  %   \end{tabular}
  % }
   \captionof{figure}{\textbf{Effect of number of iterative refinement steps.} Increasing the number of iterations of video restoration and 3D optimization steps results in more vivid details. However, the gain is negligible after a certain point. Hence, we perform 3 iterations in our experiments.
   }
   \label{fig:restoration_iteration}
\end{table}

==> figures/qualitative_over_scenes.tex <==
\begin{figure}[ht!]
  \centering
  % \includegraphics[width=\linewidth]{figures/qualitative_comparison}
  % \vspace{-2em}
  % \setlength\tabcolsep{0.1em}
  % \resizebox{\linewidth}{!}
  % {
  %   \begin{tabular}{ccccc}
  %       \includegraphics[width=.195\linewidth]{figures/qualitative_comparison/low_res/broc_low.png} 
  %       & \includegraphics[width=.195\linewidth]{figures/qualitative_comparison/in2n/broc_ing2g.png} 
  %       & \includegraphics[width=.195\linewidth]{figures/qualitative_comparison/super_nerf/broc_super_nerf.png} 
  %       & \includegraphics[width=.195\linewidth]{figures/qualitative_comparison/prehoc_img/broc_image.png} 
  %       & \includegraphics[width=.195\linewidth]{figures/qualitative_comparison/prehoc_video/broc_video.png}   \\
  %       % & \includegraphics[width=.16\linewidth]{figures/qualitative_comparison/ours/broc_ours.png} \\ 
  %       \includegraphics[width=.195\linewidth]{figures/qualitative_comparison/low_res/shoe_low.png}
  %       & \includegraphics[width=.195\linewidth]{figures/qualitative_comparison/in2n/shoe_ing2g.png} 
  %       & \includegraphics[width=.195\linewidth]{figures/qualitative_comparison/super_nerf/shoe_super_nerf.png} 
  %       & \includegraphics[width=.195\linewidth]{figures/qualitative_comparison/prehoc_img/shoe_image.png} 
  %       & \includegraphics[width=.195\linewidth]{figures/qualitative_comparison/prehoc_video/shoe_video.png} \\
  %       % & \includegraphics[width=.16\linewidth]{figures/qualitative_comparison/ours/shoe_ours.png}  \\
  %       \includegraphics[width=.195\linewidth]{figures/qualitative_comparison/low_res/hat_low.png}
  %       & \includegraphics[width=.195\linewidth]{figures/qualitative_comparison/in2n/hat_ing2g.png} 
  %       & \includegraphics[width=.195\linewidth]{figures/qualitative_comparison/super_nerf/hat_super_nerf.png} 
  %       & \includegraphics[width=.195\linewidth]{figures/qualitative_comparison/prehoc_img/hat_image.png} 
  %       & \includegraphics[width=.195\linewidth]{figures/qualitative_comparison/prehoc_video/hat_video.png} \\
  %       % & \includegraphics[width=.16\linewidth]{figures/qualitative_comparison/ours/hat_ours.png}  \\
  %       \includegraphics[width=.195\linewidth]{figures/qualitative_comparison/low_res/tiger_low.png}
  %       & \includegraphics[width=.195\linewidth]{figures/qualitative_comparison/in2n/tiger_ing2g.png} 
  %       & \includegraphics[width=.195\linewidth]{figures/qualitative_comparison/super_nerf/tiger_super_nerf.png} 
  %       & \includegraphics[width=.195\linewidth]{figures/qualitative_comparison/prehoc_img/tiger_image.png} 
  %       & \includegraphics[width=.195\linewidth]{figures/qualitative_comparison/prehoc_video/tiger_video.png} \\
  %       % & \includegraphics[width=.16\linewidth]{figures/qualitative_comparison/ours/tiger_ours.png} \\ 
  %       \includegraphics[width=.195\linewidth]{figures/qualitative_comparison/low_res/bag_low.png}
  %       & \includegraphics[width=.195\linewidth]{figures/qualitative_comparison/in2n/bag_ing2g.png} 
  %       & \includegraphics[width=.195\linewidth]{figures/qualitative_comparison/super_nerf/bag_super_nerf.png} 
  %       & \includegraphics[width=.195\linewidth]{figures/qualitative_comparison/prehoc_img/bag_image.png} 
  %       & \includegraphics[width=.195\linewidth]{figures/qualitative_comparison/prehoc_video/bag_video.png} \\
  %       % & \includegraphics[width=.16\linewidth]{figures/qualitative_comparison/ours/bag_ours.png} \\
  %       Low-res & Instruct-G2G & SuperNeRF & Pre-hoc Img  & \textbf{Ours}  \\
        
  %   \end{tabular}
  % }
  \includegraphics[width=\linewidth]{figures/qualitative_comparison_eccv}
   \vspace{-5mm}
   \captionof{figure}{\textbf{Qualitative results over upsampling scene-based 3D input.} Each column represents different poses, and each row for different scenes.
   % For each low-res 3D input (first column), we compare our method to various baselines. Given a state-of-the-art image upsampler such as GigaGAN~\cite{Kang2023GigaGAN}, \emph{Instruct-G2G} iteratively performs single frame upsampling and 3D optimization, whereas \emph{Pre-hoc image} (w/ GigaGAN) first upsamples multiple frames individually and performs a single 3D optimization. \emph{Pre-hoc video} is similar to the second baseline but upsamples the frames using the BasicVSR++ video upsampler instead. %All perform $8\times$ upsampling from $128\times128$ to $1024\times1024$. 
   % Our approach, which combines video upsampling with iterative refinement via video restoration and 3D optimization, produces richer details and eliminates certain artifacts (e.g., the boundary around the white region of the truck in the first row, ropes around the crabs in the third row.) Zoom in to appreciate the differences and check our supplementary website for an interactive qualitative comparison.
   }
   \label{fig:qual_over_scene}
   \vspace{-1.5em}
\end{figure}

==> tables/ablation_over_different_upsampling_strategies.tex <==
\begin{table*}[hbt!]
\centering
% \setlength\tabcolsep{4pt}
\def\arraystretch{1.28}
{
\small
\scalebox{0.92}{
        \hskip0em\begin{tabular}{c|cccc|cccc|cccc}
        \specialrule{.2em}{.1em}{.1em}
        % 
        & \multicolumn{4}{c|}{\textbf{Bilinear downsampled Images}}  & \multicolumn{4}{c|}{\textbf{Low-res Gaussian Splatting}~\cite{kang2023gigagan}} & \multicolumn{4}{c}{\textbf{Low-res NeRF}~\cite{tancik2023nerfstudio}}  \\
         % \cmidrule[0.5pt](lr){2-4} \cmidrule[0.5pt](lr){5-7}
          Method & LPIPS $\downarrow$ & NIQE $\downarrow$ & FID $\downarrow$ & PSNR $\uparrow$ & LPIPS $\downarrow$ & NIQE $\downarrow$ & FID $\downarrow$ & PSNR $\uparrow$ & LPIPS $\downarrow$ & NIQE $\downarrow$ & FID $\downarrow$ & PSNR $\uparrow$ \\ \hline
          Optimize over low-res images & 0.4813 & 10.7806 & 54.29 & 26.75 & 0.4817 & 10.7794 & 54.45 & 26.73 & 0.4865 & 10.8142 & 47.87 & 26.57 \\  \hline
          Pre-hoc image upsampling with hat~\cite{Chen2023Activating} & 0.3493 & 8.9832 & 23.12 & \textbf{29.03} & 0.4347 & 9.6065 & 46.92 & \textbf{27.14} & 0.4178 & 9.5997 & 33.21 & \textbf{27.35} \\
          Pre-hoc image upsampling with gigagan~\cite{Kang2023GigaGAN} & \textbf{0.3137} & \ul{7.6681} & 20.96 & \ul{28.65} & 0.3990 & 8.1391 & 43.57 & 26.93 & 0.3655 & \textbf{7.3690} & 28.20 & \ul{27.21} \\
          Iterative opt. with image prior gigagan~\cite{Kang2023GigaGAN} \\ 
          Pre-hoc video upsampling & \ul{0.3393} & \textbf{7.3815} & 30.14 & 26.27 & \textbf{0.3924} & \textbf{7.3067} & 55.84 & 24.66 & \textbf{0.3631} & \ul{7.5805} & 32.55 & 25.72\\ \hline
          % Iterative optimization with video prior \\ 
          % Pre-hoc video (fine-tuned with regression loss) & 0.3286 & 8.0807 & 28.41 & 28.13 & 0.3946 & 8.6707 & 46.02 & 26.28 & 0.3726 & 8.5829 & 33.11 & 27.02\\ 
          Pre-hoc video (fine-tuned) & \\ 
          \textbf{Ours} \\ 
        \specialrule{.1em}{.05em}{.05em}
        \end{tabular}
}
}
\caption{{\bf Ablation over up-sampling strategies on MV-ImageNet dataset}
}
\label{tab:benchmark-metrics_3}
\end{table*}

==> tables/ablation_over_different_upsampling_strategies_over_novel_trajectories.tex <==
\begin{table*}[hbt!]
\centering
% \setlength\tabcolsep{4pt}
\def\arraystretch{1.28}
{
\small
\scalebox{0.9}{
        \hskip0em\begin{tabular}{cc|cccc|cccc|cccc}
        \specialrule{.2em}{.1em}{.1em}
        % 
        & & \multicolumn{4}{c|}{\textbf{\# trajectory = 2}}  & \multicolumn{4}{c|}{\textbf{\# trajectory = 4}} & \multicolumn{4}{c}{\textbf{\# trajectory = 8}}  \\
         % \cmidrule[0.5pt](lr){2-4} \cmidrule[0.5pt](lr){5-7}
          Method & Prior & LPIPS $\downarrow$ & NIQE $\downarrow$ & FID $\downarrow$ & PSNR $\uparrow$ & LPIPS $\downarrow$ & NIQE $\downarrow$ & FID $\downarrow$ & PSNR $\uparrow$ & LPIPS $\downarrow$ & NIQE $\downarrow$ & FID $\downarrow$ & PSNR $\uparrow$ \\ \hline
          Iterative image upsampling & GigaGAN~\cite{Kang2023GigaGAN} & \\ 
          Pre-hoc image upsampling & GigaGAN~\cite{Kang2023GigaGAN} &  \\ \hline
          Iterative video upsampling & RealBasicVSR~\cite{Chan2022Investigating} & \\
          Pre-hoc image upsampling & RealBasicVSR~\cite{Chan2022Investigating} & 0.3127 & 7.56 & & 23.94 & 0.3211 & 7.69 & & 23.51 & 0.3225 & 8.09 & & 23.72 \\
          Pre-hoc video upsampling & RealBasicVSR~\cite{Chan2022Investigating} & 0.2970 & 7.08 & & 23.94 & 0.3076 & 7.30 & & 23.52\\ \hline
          Iterative video upsampling & BasicVSR++~\cite{Chan2022BasicVSR++} &  \\
          Pre-hoc image upsampling & BasicVSR++~\cite{Chan2022BasicVSR++} & 0.3001 & 8.52 & & 25.79 & 0.3062 & 8.50 & & 25.23 & 0.3099 & 8.83 & & 25.58  \\
          Pre-hoc video upsampling & BasicVSR++~\cite{Chan2022BasicVSR++} & 0.2893 & 8.16 & & 25.72 & 0.2963 & 8.19 & & 25.19 & 0.2978 & 8.39 & & 25.51 \\ \hline
          Pre-hoc video (finetuned) & BasicVSR++~\cite{Chan2022BasicVSR++} & \\ 
          \textbf{Ours} \\ 
        \specialrule{.1em}{.05em}{.05em}
        \end{tabular}
}
}
\caption{{\bf Ablation over up-sampling strategies on MV-ImageNet dataset}
}
\label{tab:benchmark-metrics_1}
\end{table*}

==> tables/ablation_over_image_conditioning.tex <==
\begin{table}[ht!]
\centering
% \setlength\tabcolsep{4pt}
\def\arraystretch{1.28}

\scriptsize
%\scalebox{0.75}{
    %\hskip0em
    \begin{tabularx}{0.7\textwidth}{c|S[table-format=1.4]S[table-format=2.2]S[table-format=2.2]{S[table-format=2.2]}} %{c|cccccc}
        \specialrule{.1em}{.1em}{.1em}
          {Upsampling Method} & \cc{LPIPS $\downarrow$} & \cc{NIQE $\downarrow$} & \cc{FID $\downarrow$} & {IS $\uparrow$}  \\ \hline
          Low-res & 0.3563 & 10.77 & 62.33 & 8.09 {~$\pm$ 0.53} \\ 
          Ours & 0.1295 & 6.84 & 24.32 & 11.09 {~$\pm$ 1.52}\\  
          Ours w/ upsampled images~ & \bfseries 0.1276 & \bfseries 6.74 & \bfseries 24.00 & \bfseries 12.07 {~$\pm$ \textbf{1.49}} \\ 
        \specialrule{.05em}{.05em}{.05em}
    \end{tabularx}
    \vspace{2mm}
%}
\caption{{\bf Ablation on incorporating upsampled images by image prior}. In the third row, we first run image upsampling on the low-res frames, and then feed both those upsampled images and the low-res frames to video upsampler. Both model setups of the second and third rows are finetuned for 100k steps. Evaluation is conducted in 3D on MV-ImgNet following our protocol.
}
\label{tab:ablation_on_condition}
\end{table}


==> tables/ablation_over_number_of_video_restoration.tex <==
\begin{table}[t]

\centering
% \setlength\tabcolsep{4pt}
\def\arraystretch{1.28}

{
\small
\scalebox{0.9}{
        \hskip-1em\begin{tabular}{c|cccc}
        \specialrule{.2em}{.1em}{.1em}
         \# iteration & LPIPS $\downarrow$ & NIQE $\downarrow$ & FID $\downarrow$ & IS $\uparrow$  \\ \hline
         0 & 0.0694 & 12.36 &  \textbf{36.34} & 10.24 $\pm$ 0.65 \\
         1 & \textbf{0.0689} & 12.09 & 37.11 & 10.43 $\pm$ 1.02 \\
         2 & 0.0713 & 11.75 & 38.47 & \textbf{10.46} $\pm$ \textbf{0.99} \\
         3 & 0.0756 & 11.41 & 40.22 & 10.29 $\pm$ 0.85 \\
         4 & 0.0810 & \textbf{11.10} & 42.26 & 10.07 $\pm$ 0.76 \\
        \specialrule{.1em}{.05em}{.05em}
        \end{tabular}}
}
% \vspace{-2mm}
\caption{{\bf Ablation over the number of video restoration iterations.} 
 }
\label{tab:ablation_over_number_of_video_restoration}
\end{table}


==> tables/ablation_over_ours_on_basicvsr.tex <==
\begin{table}[b!]
\centering
% \setlength\tabcolsep{4pt}
\def\arraystretch{1.28}
{
\small
\scalebox{0.9}{
        \hskip0em
        \begin{tabular}{c|cccccc}
        \specialrule{.2em}{.1em}{.1em}
          Method & LPIPS $\downarrow$ & NIQE $\downarrow$ & FID $\downarrow$ & IS $\uparrow$  \\ \hline
          GS over low-res & 0.0909 & 14.01 & 38.61 & 9.21 $\pm$ 0.74 \\  \hline
          %Iter video w/ upsample prior & 0.0854 & 13.65 & 39.32 & 9.61 $\pm$ 0.84 \\
          Pre-hoc video (pre-trained) & 0.0715 & 12.20  & 36.71 & 10.06 $\pm$ 0.76 \\ 
          Pre-hoc video (fine-tuned) & 0.0694 & 12.36 & \textbf{36.34} & 10.24 $\pm$ 0.65 \\
          \textbf{Ours} & \textbf{0.0689} & \textbf{12.09} & 37.11 & \textbf{10.46} $\pm$ \textbf{0.99} \\ 
        \specialrule{.1em}{.05em}{.05em}
        \end{tabular}
}
}
\caption{{\bf Quantitative ablations}. We evaluate the effect of the additional finetuning of the video upsampler to adapt to specific degradations of Gaussian splats and the usefulness of the iterative refinement via the video restoration module. We report the quantitative metrics on the low-res inputs as well to provide a point of reference. Our full pipeline yields the best results verifying the design choices we have made.
}
\label{tab:ablation}
\vspace*{-.1in}
\end{table}





% \begin{table*}[hbt!]
% \centering
% % \setlength\tabcolsep{4pt}
% \def\arraystretch{1.28}
% {
% \small
% \scalebox{0.9}{
%         \hskip0em\begin{tabular}{cc|cccccc|cccccc}
%         \specialrule{.2em}{.1em}{.1em}
%         % 
%         &  & \multicolumn{6}{c|}{\textbf{Gaussian Splatting}~\cite{Kang2023GigaGAN}} & \multicolumn{6}{c}{\textbf{NeRF}~\cite{Tancik2023NeRFStudio}}  \\
%          % \cmidrule[0.5pt](lr){2-4} \cmidrule[0.5pt](lr){5-7}
%           Method & Prior & LPIPS $\downarrow$ & NIQE $\downarrow$ & FID $\downarrow$ & IS $\uparrow$ & PSNR $\uparrow$ & FS$\uparrow$ & LPIPS $\downarrow$ & NIQE $\downarrow$ & FID $\downarrow$ & IS $\uparrow$ & PSNR $\uparrow$ & FS$\uparrow$  \\ \hline
%           Optimize over low-res images & - & 0.3593 & 11.20 & 57.10 & 10.40 $$\pm$$ 0.62 & 27.15 \\  \hline
%           Iterative image upsampling & GigaGAN~\cite{Kang2023GigaGAN} & \\ 
%           Pre-hoc image upsampling & GigaGAN~\cite{Kang2023GigaGAN} & 0.2697 & 8.47 & 46.09 & 11.69 $$\pm$$ 1.60 & 27.24 \\ \hline
%           Iterative video upsampling & RealBasicVSR~\cite{Chan2022Investigating} & \\
%           Pre-hoc image upsampling & RealBasicVSR~\cite{Chan2022Investigating} & 0.3054 & 8.23 & 67.82 & 8.97 $$\pm$$ 0.59 & 24.67 \\
%           Pre-hoc video upsampling & RealBasicVSR~\cite{Chan2022Investigating} & 0.2935 & 7.63 & 64.23 & 9.81 $$\pm$$ 1.42 & 24.62 \\ \hline
%           Iterative video upsampling & BasicVSR++~\cite{Chan2022BasicVSR++} & 0.3249 & 10.01 & 51.82 & 10.73 $$\pm$$ 0.99 & 25.68 \\
%           Pre-hoc image upsampling & BasicVSR++~\cite{Chan2022BasicVSR++}  & 0.2936 & 9.54 & 49.31 & 10.70 $$\pm$$ 1.18 & 27.46 \\
%           Pre-hoc video upsampling & BasicVSR++~\cite{Chan2022BasicVSR++} & \\ 
%           Pre-hoc video upsampling (fine-tuned) & BasicVSR++~\cite{Chan2022BasicVSR++} & 0.2619 & 9.09 & 20.51 & 14.07 $$\pm$$ 1.25 & 27.55 \\ \hline
%           \textbf{Ours} & BasicVSR++~\cite{Chan2022BasicVSR++} & \\ 
%         \specialrule{.1em}{.05em}{.05em}
%         \end{tabular}
% }
% }
% \caption{{\bf Ablation over up-sampling strategies on MV-ImageNet dataset}
% }
% \label{tab:benchmark-metrics_2}
% \end{table*}

==> tables/ablation_over_prior_types.tex <==
\begin{table}[t]
\centering
\def\arraystretch{1.28}
\caption{{\bf Ablation on which prior type is better for 3D upsampling purpose}. The only difference between the above is the used prior type. Both cases upsample at frame level and then perform 3D reconstruction. Studies are conducted on MV-ImgNet.
}
{
\scriptsize
\begin{tabularx}{0.65\textwidth}{c|S[table-format=1.4]S[table-format=1.2]S[table-format=2.2]S[table-format=2.2]}
    \specialrule{.1em}{.1em}{.1em}
      {Upsampling Method} & {~LPIPS $\downarrow$~} & {~NIQE $\downarrow$~} & {~FID $\downarrow$~} & {~IS $\uparrow$~}  \\ \hline
      Pre-hoc image & 0.1531 & 7.70 & 27.04 & 10.72 {~$\pm$ 0.89} \\
      Pre-hoc video & \bfseries 0.1295 & \bfseries 6.84 & \bfseries 24.32 & \bfseries 11.09 {~$\pm$ \textbf{1.52}} \\  
    \specialrule{.05em}{.05em}{.05em}
\end{tabularx}
\vspace{2mm}
}
\label{tab:prior_type_ablation}
\vspace{-1.5em}
\end{table}

==> tables/ablation_studies/01_video_and_image.tex <==
\begin{table}[b!]
\centering
% \setlength\tabcolsep{4pt}
\def\arraystretch{1.28}
{
\small
\scalebox{0.9}{
        \hskip0em
        \begin{tabular}{c|cccccc}
        \specialrule{.2em}{.1em}{.1em}
          Method & LPIPS $\downarrow$ & NIQE $\downarrow$ & FID $\downarrow$ & IS $\uparrow$  \\ \hline
           & 0.0909 & 14.01 & 38.61 & 9.21 $\pm$ 0.74 \\  \hline
          %Iter video w/ upsample prior & 0.0854 & 13.65 & 39.32 & 9.61 $\pm$ 0.84 \\
          Pre-hoc video (pre-trained) & 0.0715 & 12.20  & 36.71 & 10.06 $\pm$ 0.76 \\ 
          Pre-hoc video (fine-tuned) & 0.0694 & 12.36 & \textbf{36.34} & 10.24 $\pm$ 0.65 \\
          \textbf{Ours} & \textbf{0.0689} & \textbf{12.09} & 37.11 & \textbf{10.46} $\pm$ \textbf{0.99} \\ 
        \specialrule{.1em}{.05em}{.05em}
        \end{tabular}
}
}
\caption{{\bf Quantitative ablations}. We evaluate the effect of the additional finetuning of the video upsampler to adapt to specific degradations of Gaussian splats and the usefulness of the iterative refinement via the video restoration module. We report the quantitative metrics on the low-res inputs as well to provide a point of reference. Our full pipeline yields the best results verifying the design choices we have made.
}
\label{tab:ablation}
\vspace*{-.1in}
\end{table}


==> tables/comparison_with_sota.tex <==
% \begin{table}[t!]
% \centering
% % \setlength\tabcolsep{4pt}
% \def\arraystretch{1.28}
% {
% \scriptsize
% %\scalebox{0.8}{
%         \begin{tabularx}{0.7\textwidth}{cc|S[table-format=1.3]S[table-format=2.2]S[table-format=1.3]}
%         \specialrule{.1em}{.1em}{.1em}
%           Upsampling Scale & Method  & {~LPIPS $\downarrow$~} & {~PSNR $\uparrow$~} & {~SSIM $\uparrow$~}  \\ \hline
%           \multirow{2}{*}{$\times$ 1~~} & NeRF~\cite{Mildenhall2021NeRF} & 0.250 & 26.5 & 0.811 \\ 
%            & TensoRF~\cite{chen2022tensorf}  & 0.207 & 26.6 & 0.832 \\ \hline
%          \multirow{2}{*}{$\times$ 2~~} & FastSR-NeRF~\cite{Lin2024FastSR} & 0.241 & 26.20 & 0.822 \\
%           &  Ours w/ TF &  \bfseries 0.131 & \bfseries 27.14 & \bfseries 0.853\\ \hline
         
%           \multirow{2}{*}{$\times$ 4~~} & FastSR-NeRF~\cite{Lin2024FastSR} & 0.297 & 25.41 & 0.784 \\
%           &  Ours w/ TF & \bfseries 0.210 & \bfseries 25.47 & 0.784  \\ \hline
          
%           \multirow{2}{*}{$\times$ 8~~} & FastSR-NeRF~\cite{Lin2024FastSR} & 0.475 & 21.30  & 0.584 \\ 
%           &  Ours w/ TF & \bfseries 0.335 & \bfseries 22.48 & \textbf{0.645} \\
%         \specialrule{.05em}{.05em}{.05em}
%         \end{tabularx}
% %}
% }
% \vspace{1em}
% \caption{{\bf Quantitative Comparison on NeRF LLFF dataset to upsample low-res posed RGB images.} We follow the experiment protocol in FastSR-NeRF by setting the target resolution at $1008\times 756$. For fair comparison, we use TensoRF in the 3D reconstruction step as other baselines. In ours, one off-the-shelf video upsampler, RealBasicVSR, is used, which is pre-trained on REDS dataset. FastSR-NeRF~\cite{Lin2024FastSR} results are directly obtained from their Table 1.
% }
% \vspace{-1.5em}
% \label{tab:benchmark-metrics_4}
% \end{table}


\begin{table}[t]
\centering
\setlength\tabcolsep{3.5pt}
\def\arraystretch{1.28}
{
\scriptsize
%\scalebox{0.8}{
\begin{tabularx}{0.53\textwidth}{c|S[table-format=1.4]S[table-format=1.2]S[table-format=1.4]}
    \specialrule{.1em}{.1em}{.1em}
        %\hskip0em\begin{tabular}{c|ccccccc}
        %\specialrule{.2em}{.1em}{.1em}
      Method & {LPIPS $\downarrow$} & {PSNR $\uparrow$} & {SSIM $\uparrow$} \\ \hline
      FastSR-NeRF~\cite{Lin2024FastSR} & 0.075 & \bfseries 30.47 & \bfseries 0.944 \\ 
      NeRF-SR~\cite{Wang2022NeRFSR} & 0.076 & 28.46 & 0.921 \\  
      Ours & \bfseries 0.067 & 28.44 & 0.923 \\ 
      % Ours + Refinement & 0.1505 & \textbf{6.75} & 30.31 & 11.07 $\pm$ 0.75 \\
    \specialrule{.05em}{.05em}{.05em}
    \end{tabularx}
}
%}
\vspace{1em}
\caption{{\bf Quantitative Comparison on Blender synthetic dataset to upsample low-res posed RGB images}. Here, we compare on $\times 4$ upsampling from $200\times200$ to $800\times800$px. We compare our methods against baselines on the official test set using metrics reported in prior work. Our method produces on-par quantitative results. Besides, our results yield more generative details, which are not captured by the reference metrics. For a fair comparison, we use Neural Radiance Field, i.e., TensoRF~\cite{chen2022tensorf}, as our 3D representation. Other baseline results are directly taken from their paper.
}
\vspace{-1.5em}
\label{tab:benchmark-metrics_5}
\end{table}



